GlobEnc: Quantifying Global Token Attribution by Incorporating the Whole Encoder Layer in Transformers

There has been a growing interest in interpreting the underlying dynamics of Transformers. While self-attention patterns were initially deemed as the primary option, recent studies have shown that integrating other components can yield more accurate explanations. This paper introduces a novel token attribution analysis method that incorporates all the components in the encoder block and aggregates this throughout layers. Through extensive quantitative and qualitative experiments, we demonstrate that our method can produce faithful and meaningful global token attributions. Our experiments reveal that incorporating almost every encoder component results in increasingly more accurate analysis in both local (single layer) and global (the whole model) settings. Our global attribution analysis significantly outperforms previous methods on various tasks regarding correlation with gradient-based saliency scores. Our code is freely available at https://github.com/mohsenfayyaz/GlobEnc.

==> plots/sst2_hta_swap_beginning.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.49\textwidth]{./figures/sst2_HTA_swap_beginning_95.pdf}
    \caption{Spearman correlation of saliency scores with aggregated attribution scores where the complete 12-layer HTA attribution map is replaced with the corresponding method's attribution map from the begining to the indicated layer. The \red{95\% confidence} interval is drawn in the plot. 
    }
    \label{fig:sst2_htw_swap_beginning}
\end{figure}
